Optimal Stopping with Randomly Arriving Stopping Opportunities

We develop simulation-based methods to solve general optimal stopping problems with opportunities to stop that arrive randomly. Such problems occur naturally in a wide variety of applications with market frictions, such as limited liquidity, incomplete information and transaction costs. Our approach employs random time scales to map the original problem to an integer-time stopping problem with (possibly) infinite horizon. We introduce an infinite-horizon policy iteration algorithm to generate lower-biased estimates of the value function and establish a martingale dual representation to generate upper-biased estimates. Furthermore, we extend a family of backward dynamic programming methods that includes least-squares Monte Carlo. We illustrate the performance of our methods, their general applicability and the managerial implications of randomly arriving opportunities to stop in three examples: a stopped jump-diffusion that can be analyzed in closed form, a random-exercise version of a multi-dimensional max-call contract, and a real options problem in an illiquid market.

==> literature_overview.tex <==
\subsection{Examples of (applications of) optimal stopping on random times in the literature}
\todo[inline]{Om te voorkomen dat we op een later moment belangrijke verwijzingen missen, begin ik hier met een overzicht van belangrijke referenties.}

\subsubsection{Theory}
{\color{red} \paragraph{Hobson and Zeng (2022) \cite{HZ22}}
They extend upon Hobson (2021) by allowing the arrival rate of opportunities to be controllable. 
\paragraph{Hobson (2021) \cite{H21}}
They consider the problem of an inhomogeneous Poisson process with state-dependent arrivals. 
\begin{itemize}
    \item They provide theoretical shape results for Brownian-driven dynamics. 
    \item See Liang, Lütkebohmert, Wei (2015) for an application that already involved state-dependent arrivals. 
\end{itemize}}

{\color{red} \paragraph{Menaldi and Robin (2016) \cite{MR16}}
Generalize the set-up of \cite{L12} to Markov-Feller processes, general point processes and indicate how state-dependent arrivals may be introduced. }

{\color{blue} \paragraph{Liang and Wei (2016) \cite{LW16}}
Generalizes the set-up of \cite{DW02}, \cite{L12} and Liang, Lütkebohmert and Wei (2015) to optimal switching. 
\begin{itemize}
    \item They indicate that the Poisson process may be interpreted as a limited liquidity or information constraint
\end{itemize}}

{\color{blue} \paragraph{Lempa (2012) \cite{L12}}
Generalizes the set-up of \cite{DW02} to more general payoff and dynamics. }

{\color{red} \paragraph{Egloff and Leippold (2009) \cite{EL09}}
Rather than allowing stopping on random times, they allow stopping while the state process is in some active set. Not a generalization, but may be interesting to mention? }

{\color{blue} \paragraph{Dupuis and Wang (2002) \cite{DW02}}
They consider the problem of optimally stopping a perpetual American option on independent Poisson opportunities and are the first in the literature to do so. They use these to model illiquidity, which is similar to what \cite{DW02} do. }

{\color{blue} \paragraph{Rogers and Zane (2002) \cite{RZ02}}
They consider an optimal consumption and investment problem on independent Poisson opportunities and are the first in the literature to do so. They use these to model illiquidity, which is similar to what \cite{DW02} do. }

\subsubsection{Real options}
{\color{blue} \paragraph{Lange, Ralph and Støre (2020) \cite{LRS20}, Lange and Teulings (2021) \cite{LT21}}
They consider the valuation of real options using Poisson optional stopping times, which serves as an approximation technique for the American option pricing problem but also has an interpretation as a limited-liquidity/random-times real option value problem. 
\begin{itemize}
    \item They provide a finite-difference scheme. (Note that there will be a follow-up paper with more mathematical details!)
\end{itemize}}

\subsubsection{Limited liquidity/information constraint}
{\color{blue} \paragraph{Dupuis and Wang (2002) \cite{DW02}, Rogers and Zane (2002) \cite{RZ02}}
Both consider independent Poisson opportunities as a model for limited liquidity. }

\subsubsection{Information constraint}
{\color{blue} \paragraph{Lempa (2012) \cite{L12}}
Considers Poisson arriving stopping opportunities as either a ``randomized Bermudan'' or as a model for limited information, following \cite{GL05}. 

\paragraph{Guo and Liu (2005) \cite{GL05}}
Consider Poisson arriving stopping opportunities as a model for limited information. }

\subsubsection{Debt runs}
{\color{red} \paragraph{Liang, Lütkebohmert and Wei (2015) \cite{LLW15}}
They model the problem of the representative short-run creditor as an optimal stopping problem on random times. 
\begin{itemize}
    \item The decision whether or not debt may be rolled over is made at (possibly randomly arriving) short-term debt maturity dates. 
    \item Earlier literature used deterministic/Poisson arriving short-term debt maturity dates, this article also allow for a state-dependent Cox process. 
\end{itemize}}

{\color{blue} \paragraph{He and Xiong (2012) \cite{HX12}}
They consider the problem of dynamic debt runs as a coordination problem: short-term credit matures at a Poisson rate, at which point the credit must decide to roll-over the debt or to run, thus giving an optimal stopping problem on random times (the successive maturities of the credits supplied by this creditor). The solutions to this problem are then used to solve a coordination problem among credits, to determine whether they perform a debt run. They follow the staggered-pricing model of  Calvo (1983) and the credit-risk Leland (1998) in modeling debt contracts as lasting for a random period. \todo{Are these interesting to mention as early examples of problems in which considering random timings is natural? }}


==> results/poisson_dependent_2.tex <==
\begin{tabular}{rr|rrrrrrrr}
$\lambda$ & $X_0$ & LSMC & (s.e.) & Dual & (s.e.) & Threshold & (s.e.) & PI-threshold & (s.e.) \\\hline 
1 & 90.0 & 3.07576 & 0.00586 & 3.07771 & 0.00073 & 3.02144 & 0.00571 & 3.09369 & 0.02614 \\
1 & 100.0 & 7.70795 & 0.00889 & 7.71086 & 0.00101 & 7.54196 & 0.00866 & 7.67702 & 0.03934 \\
1 & 110.0 & 14.70432 & 0.01147 & 14.70606 & 0.00060 & 14.35433 & 0.01096 & 14.69009 & 0.05128 \\
3 & 90.0 & 4.35653 & 0.00655 & 4.36299 & 0.00223 & 4.14472 & 0.00612 & 4.39281 & 0.02885 \\
3 & 100.0 & 10.17052 & 0.00936 & 10.17567 & 0.00123 & 9.60816 & 0.00877 & 10.14695 & 0.04021 \\
3 & 110.0 & 18.30373 & 0.01157 & 18.31253 & 0.00175 & 17.30562 & 0.01046 & 18.22435 & 0.04830 \\
5 & 90.0 & 4.75333 & 0.00674 & 4.76532 & 0.00325 & 4.46660 & 0.00622 & 4.76585 & 0.02885 \\
5 & 100.0 & 10.84360 & 0.00943 & 10.88247 & 0.02240 & 10.14199 & 0.00859 & 10.76841 & 0.03888 \\
5 & 110.0 & 19.15250 & 0.01149 & 19.17718 & 0.00511 & 17.94741 & 0.01043 & 18.99140 & 0.04596 \\
\end{tabular}


==> results/poisson_dependent_5.tex <==
\begin{tabular}{rr|rrrrrrrr}
$\lambda$ & $X_0$ & LSMC & (s.e.) & Dual & (s.e.) & Threshold & (s.e.) & PI-threshold & (s.e.) \\\hline 
1 & 90.0 & 1.35781 & 0.00376 & 1.35982 & 0.00100 & 1.35565 & 0.00375 & 1.37197 & 0.01712 \\
1 & 100.0 & 7.25039 & 0.00815 & 7.26267 & 0.00331 & 7.19173 & 0.00808 & 7.29730 & 0.03693 \\
1 & 110.0 & 17.27549 & 0.01225 & 17.29726 & 0.00567 & 17.00855 & 0.01201 & 17.30077 & 0.05565 \\
3 & 90.0 & 2.37091 & 0.00458 & 2.39623 & 0.00589 & 2.35055 & 0.00452 & 2.39509 & 0.02049 \\
3 & 100.0 & 10.80182 & 0.00843 & 10.95147 & 0.01677 & 10.52893 & 0.00812 & 11.03803 & 0.03840 \\
3 & 110.0 & 23.06813 & 0.01142 & 23.51275 & 0.03848 & 22.14128 & 0.01108 & 23.66928 & 0.05089 \\
5 & 90.0 & 2.82667 & 0.00480 & 2.87871 & 0.00778 & 2.78262 & 0.00475 & 2.90619 & 0.02191 \\
5 & 100.0 & 11.99038 & 0.00835 & 12.43954 & 0.05010 & 11.57660 & 0.00804 & 12.39019 & 0.03712 \\
5 & 110.0 & 24.65389 & 0.01112 & 25.64435 & 0.06160 & 23.49051 & 0.01057 & 25.41821 & 0.04733 \\
\end{tabular}

